Spin gauge symmetry in the action principle for classical relativistic particles

We suggest that the physically irrelevant choice of a representative worldline of a relativistic spinning particle should correspond to a gauge symmetry in an action approach. Using a canonical formalism in special relativity, we identify a (first-class) spin gauge constraint, which generates a shift of the worldline together with the corresponding transformation of the spin on phase space. An action principle is formulated for which a minimal coupling to fields is straightforward. The electromagnetic interaction of a monopole-dipole particle is constructed explicitly.

==> fig1_code.tex <==
\begin{tikzpicture}[semithick]
\draw[->,red] (0,1.5) node[above]{fast and heavy} -- (-1.5,1.5);
\draw[->,red] (0,-1.5) node[below]{slow and light} -- (0.7,-1.5);
\draw[->,red] (0,0) -- (0,0.25) node[right]{$\Delta z^i$} -- (0,0.5);
\draw (0,0) circle (1.5);
\draw[|->] (0,0) -- (-0.35,0) node[above,black]{$v^i$} -- (-0.7,0);
\draw[->] (-140:0.7) arc (-140:-90:0.7) node[below]{spin} arc (-90:-40:0.7);
\end{tikzpicture}

